Route Anything: A Study of Model and Policy Routing for General-Purpose AI Systems

Artificial general intelligence (AGI) requires a method that can understand, generate, reason, and act across diverse domains and modalities. Rather than relying on a single model to master every capability, a promising path toward AGI now is to orchestrate a heterogeneous ecosystem of specialized models, tools, and policies (candidates) into a unified AI system. At the heart of this vision lies a fundamental question: how can an AI system dynamically select and coordinate the most capable candidate for each task while balancing performance and computational cost? In this work, we present Route Anything, a unified framework for studying model and policy routing across general-purpose AI systems. We develop a unified theoretical foundation that characterizes optimal routing under quality--cost trade-offs and establishes how the information available to a router determines its attainable performance. To systematically investigate routing across diverse capabilities, we first construct an omni-modal trajectory matrix spanning 25 benchmarks across language understanding, image, video, and speech generation, coding and workplace agents, and robotic manipulation, comprising 374,401 scored runs from 452 candidate configurations. Building on this framework, we train and test different routers to investigate the potential of omni-modal model routing, the capabilities of learned routers, and the conditions under which routing improves efficiency. Our results reveal substantial opportunities for capability orchestration: per-input oracle routing outperforms the best fixed candidate by 5.4 points, and learned routers outperform it by 0.3 points across 16 benchmarks, by 2.1 points on video generation, and by 1.1 points on robot manipulation while using 24% less policy time. More importantly, routing raises efficiency by 8.82x on average compared with the reference model.

==> fig/omni-teaser.tex <==
% Teaser: (a) one router over candidate pools of every output type; (b) headroom by modality on the
% test split (Table 1); (c) efficiency of near-zero-loss price routes (Table 4).
\begingroup
\definecolor{vizblue}{HTML}{2A78D6}%
\definecolor{vizfixed}{HTML}{86B6EF}%
\definecolor{vizoracle}{HTML}{1C5CAB}%
\definecolor{vizink}{HTML}{0B0B0B}%
\definecolor{vizmuted}{HTML}{52514E}%
\tikzset{
  chip/.style={rounded corners=2pt,font=\scriptsize,text=vizink,minimum height=0.44cm,
    inner xsep=2pt,inner ysep=1pt,align=center},
  inchip/.style={chip,draw=black!20,fill=white,minimum width=2.15cm},
  armchip/.style={chip,draw=vizblue!40,fill=white,minimum width=2.15cm},
  group/.style={rounded corners=3pt,inner sep=4pt},
  flow/.style={-{Stealth[length=3.4pt]},draw=black!45,line width=0.6pt},
  paneltitle/.style={font=\footnotesize\bfseries,text=vizink,anchor=base west},
}%
\pgfplotsset{
  teaseraxis/.style={
    scale only axis,
    axis x line*=bottom,axis y line*=left,
    y axis line style={draw=none},ytick style={draw=none},
    tick align=outside,xtick pos=bottom,
    tick label style={font=\scriptsize,text=vizmuted},
    label style={font=\scriptsize,text=vizmuted},
    yticklabel style={font=\scriptsize,text=vizink,align=right,xshift=-2pt},
    xmajorgrids,major grid style={black!9},
    axis line style={black!35},
    clip=false,
  },
}%
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}
% ---------------- (a) one router, every output type ----------------
\node[paneltitle] at (0,4.05) {(a) One router, every output type};
\foreach \y/\t [count=\k] in {3.35/{Question},2.8/{Image + question},2.25/{Task + files},
                              1.7/{Generation prompt},1.15/{Cameras + state}}
  \node[inchip] (in\k) at (1.15,\y) {\t};
\foreach \y/\t/\n [count=\k] in {3.35/{Language models}/{3--4},2.8/{Image generators}/6,
                                 2.25/{Video generators}/3,1.7/{Speech generators}/3,1.15/{Robot policies}/7}
  {\node[armchip] (arm\k) at (5.75,\y) {\t};
   \node[font=\scriptsize,text=vizmuted,anchor=west] at (arm\k.east) {$\times$\n};}
\begin{scope}[on background layer]
  \node[group,fill=black!4,fit=(in1)(in5)] (inputs) {};
  \node[group,fill=vizblue!6,fit=(arm1)(arm5)] (arms) {};
\end{scope}
\node[draw=vizblue,fill=vizblue!14,rounded corners=3pt,minimum width=1.25cm,minimum height=1.15cm,
      align=center,font=\scriptsize,text=vizink] (router) at (3.45,2.25)
      {\textbf{Router}\\[2pt]$\max_u\,v-\lambda c$};
\draw[flow] (inputs.east |- router) -- (router.west);
\draw[flow] (router.east) -- (arms.west |- router);
\node[font=\scriptsize,text=vizmuted,anchor=north] at (3.45,0.62)
  {25 benchmarks $\cdot$ 374,401 scored runs $\cdot$ 452 candidate configurations};
% ---------------- (b) headroom by modality ----------------
\node[paneltitle] at (7.95,4.05) {(b) Per-input potential gain, test split};
\begin{axis}[teaseraxis,at={(9.85cm,0.62cm)},width=2.45cm,height=2.95cm,
  xmin=60,xmax=100,xtick={60,80,100},ymin=-0.2,ymax=7.5,
  ytick={1,...,7},
  yticklabels={Robots,Agents,Speech gen.,Video gen.,Image gen.,Image-text QA,Text QA},
  xlabel={Quality, 19,814 inputs},xlabel style={yshift=3pt}]
\foreach \f/\o/\i in {70.45/88.85/1,69.17/77.29/2,98.62/99.30/3,62.43/81.36/4,
                      82.93/87.92/5,85.32/88.02/6,83.27/87.56/7}
  {\edef\temp{\noexpand\draw[black!22,line width=1.7pt]
     (axis cs:\f,\i) -- (axis cs:\o,\i);}\temp}
\addplot[only marks,mark=*,mark size=2.4pt,mark options={fill=vizfixed,draw=white,line width=0.7pt}]
  coordinates {(70.45,1) (69.17,2) (98.62,3) (62.43,4) (82.93,5) (85.32,6) (83.27,7)};
\addplot[only marks,mark=*,mark size=2.4pt,mark options={fill=vizoracle,draw=white,line width=0.7pt}]
  coordinates {(88.85,1) (77.29,2) (99.30,3) (81.36,4) (87.92,5) (88.02,6) (87.56,7)};
\foreach \o/\g/\i in {88.85/18.4/1,77.29/8.1/2,99.30/0.7/3,81.36/18.9/4,87.92/5.0/5,88.02/2.7/6,87.56/4.3/7}
  {\edef\temp{\noexpand\node[font=\noexpand\scriptsize,text=vizmuted,anchor=west,inner sep=1.5pt]
     at (axis cs:\o,\i) {\noexpand\hspace{1.6pt}+\g};}\temp}
\node[font=\scriptsize,text=vizmuted,anchor=north,inner sep=1pt] at (axis cs:70.45,0.82) {fixed};
\node[font=\scriptsize,text=vizoracle,anchor=north,inner sep=1pt] at (axis cs:88.85,0.82) {oracle};
\end{axis}
% ---------------- (c) price routes ----------------
\node[paneltitle] at (13.85,4.05) {(c) Efficiency at a $<$0.5-point loss};
\begin{axis}[teaseraxis,at={(15.65cm,0.62cm)},width=2.25cm,height=2.95cm,
  xmode=log,log basis x=10,xmin=1,xmax=100,xtick={1,3,10,30},xticklabels={1,3,10,30},
  ymin=0.4,ymax=4.6,ytick={1,...,4},
  yticklabels={Robots (s),Image gen.\ (\$),Text QA (\$),Code (\$)},
  xlabel={$\eta/\eta_B$, log scale},xlabel style={yshift=3pt}]
\foreach \v/\l/\q/\i in {1.33/1.33/{+1.1}/1,1.35/1.35/{$-$0.5}/2,7.10/7.1/{$-$0.4}/3,25.52/25.5/{$-$0.4}/4}
  {\edef\temp{\noexpand\fill[vizblue,rounded corners=1.2pt]
     (axis cs:1,\i-0.26) rectangle (axis cs:\v,\i+0.26);
   \noexpand\node[font=\noexpand\scriptsize,text=vizink,anchor=west,inner sep=1.5pt] at (axis cs:\v,\i)
     {\noexpand\hspace{1pt}\l$\noexpand\times$\noexpand\enspace{\noexpand\color{vizmuted}\q\,pt}};}\temp}
\end{axis}
\end{tikzpicture}}%
\endgroup


==> fig/policy-comparison.tex <==
% \begingroup%
% \definecolor{policyblue}{HTML}{3568A8}%
% \definecolor{policyteal}{HTML}{2A8C82}%
% \definecolor{policyslate}{HTML}{526171}%
% \definecolor{policyamber}{HTML}{BD8035}%
% \pgfplotsset{
%   policyaxis/.style={
%     scale only axis,height=5.0cm,
%     ymin=0.5,ymax=10.5,ytick={1,...,10},
%     axis x line*=bottom,axis y line*=left,
%     tick align=outside,xtick pos=bottom,
%     tick label style={font=\footnotesize,text=black!75},
%     label style={font=\footnotesize},
%     title style={font=\footnotesize\bfseries,yshift=1pt},
%     xmajorgrids,major grid style={black!10},
%     axis line style={black!35},
%     y axis line style={draw=none},
%     ytick style={draw=none},
%     clip=false,
%   },
%   policyinterval/.style={
%     only marks,mark=*,mark size=2.2pt,
%     error bars/.cd,x dir=both,x explicit,
%     error bar style={line width=0.9pt},
%     error mark options={rotate=90,mark size=2.2pt,line width=0.7pt},
%     /pgfplots/.cd,
%   },
% }%
% \resizebox{0.92\textwidth}{!}{%
% \begin{tikzpicture}
% \begin{axis}[policyaxis,name=efficiency,width=3.05cm,
%   xmode=log,log basis x=10,xmin=0.8,xmax=45,
%   xtick={1,3,10,30},xticklabels={1,3,10,30},
%   yticklabels={Always-Opus,
%     Per-task oracle,
%     ACRouter map,
%     Best fixed cascade,
%     Fixed Qwen3-Max dispatch,
%     Quality-cost router,
%     {Predicted 21 cells, $\epsilon=0$},
%     {21 cells, $\epsilon=0.01$},
%     {21 cells, $\epsilon=0$},
%     {21 cells, unconstrained}},
%   yticklabel style={font=\footnotesize,text=black!85,align=right},
%   title={Dollar efficiency},xlabel={$\eta/\eta_B$ (log scale)}]
% \path[fill=policyblue!5] (axis cs:0.8,7.5) rectangle (axis cs:45,10.5);
% \path[fill=policyteal!7] (axis cs:0.8,5.5) rectangle (axis cs:45,7.5);
% \addplot[black!45,dashed,line width=0.6pt] coordinates {(1,0.5) (1,10.5)};
% \addplot[policyinterval,color=policyblue] coordinates {
%   (28.187,10) += (1.472,0) -= (1.347,0)
%   (25.516,9) += (1.387,0) -= (1.238,0)
%   (27.612,8) += (1.460,0) -= (1.301,0)
% };
% \addplot[policyinterval,color=policyteal] coordinates {
%   (25.324,7) += (1.326,0) -= (1.227,0)
%   (24.166,6) += (1.415,0) -= (1.305,0)
% };
% \addplot[policyinterval,color=policyslate] coordinates {
%   (20.097,5) += (1.200,0) -= (1.132,0)
%   (2.004,4) += (0.136,0) -= (0.123,0)
%   (1.745,3) += (0.081,0) -= (0.079,0)
% };
% \addplot[policyinterval,color=policyamber,mark=diamond*,mark size=2.8pt]
%   coordinates {(33.510,2) += (1.696,0) -= (1.445,0)};
% \addplot[only marks,mark=square*,mark size=2.1pt,color=black!70]
%   coordinates {(1,1)};
% \end{axis}
% \begin{axis}[policyaxis,at={(efficiency.south east)},anchor=south west,xshift=0.48cm,
%   name=cost,width=2.55cm,yticklabels={},
%   xmode=log,log basis x=10,xmin=0.28,xmax=15,
%   xtick={0.5,1,3,10},xticklabels={0.5,1,3,10},
%   title={Cost per task},xlabel={m\$ (log scale)}]
% \path[fill=policyblue!5] (axis cs:0.28,7.5) rectangle (axis cs:15,10.5);
% \path[fill=policyteal!7] (axis cs:0.28,5.5) rectangle (axis cs:15,7.5);
% \addplot[black!45,dashed,line width=0.6pt] coordinates {(11.655,0.5) (11.655,10.5)};
% \addplot[only marks,mark=*,mark size=2.2pt,color=policyblue]
%   coordinates {(0.395,10) (0.452,9) (0.409,8)};
% \addplot[only marks,mark=*,mark size=2.2pt,color=policyteal]
%   coordinates {(0.453,7) (0.482,6)};
% \addplot[only marks,mark=*,mark size=2.2pt,color=policyslate]
%   coordinates {(0.525,5) (6.556,4) (7.643,3)};
% \addplot[only marks,mark=diamond*,mark size=2.8pt,color=policyamber]
%   coordinates {(0.368,2)};
% \addplot[only marks,mark=square*,mark size=2.1pt,color=black!70]
%   coordinates {(11.655,1)};
% \end{axis}
% \begin{axis}[policyaxis,at={(cost.south east)},anchor=south west,xshift=0.48cm,
%   width=3.5cm,yticklabels={},xmin=-0.065,xmax=0.083,scaled x ticks=false,
%   xtick={-0.05,0,0.05},xticklabels={$-0.05$,$0$,$+0.05$},
%   title={Quality change},xlabel={Mean score, $\Delta V$}]
% \path[fill=policyblue!5] (axis cs:-0.065,7.5) rectangle (axis cs:0.083,10.5);
% \path[fill=policyteal!7] (axis cs:-0.065,5.5) rectangle (axis cs:0.083,7.5);
% \addplot[black!45,dashed,line width=0.6pt] coordinates {(0,0.5) (0,10.5)};
% \addplot[policyinterval,color=policyblue] coordinates {
%   (-0.0201,10) += (0.0145,0) -= (0.0142,0)
%   (-0.0044,9) += (0.0141,0) -= (0.0131,0)
%   (-0.0140,8) += (0.0136,0) -= (0.0132,0)
% };
% \addplot[policyinterval,color=policyteal] coordinates {
%   (-0.0070,7) += (0.0137,0) -= (0.0130,0)
%   (-0.0003,6) += (0.0135,0) -= (0.0135,0)
% };
% \addplot[policyinterval,color=policyslate] coordinates {
%   (-0.0416,5) += (0.0141,0) -= (0.0133,0)
%   (0.0558,4) += (0.0102,0) -= (0.0097,0)
%   (0.0631,3) += (0.0100,0) -= (0.0103,0)
% };
% \addplot[policyinterval,color=policyamber,mark=diamond*,mark size=2.8pt]
%   coordinates {(0.0248,2) += (0.0128,0) -= (0.0131,0)};
% \addplot[only marks,mark=square*,mark size=2.1pt,color=black!70]
%   coordinates {(0,1)};
% \end{axis}
% \end{tikzpicture}%
% }%
% \endgroup%



\begingroup%
\definecolor{policyblue}{HTML}{3568A8}%
\definecolor{policyteal}{HTML}{2A8C82}%
\definecolor{policyslate}{HTML}{526171}%
\definecolor{policyamber}{HTML}{BD8035}%
% Layout: a label column plus three equal panels, spanning exactly \linewidth.
\newlength{\policylabelw}\settowidth{\policylabelw}{\footnotesize Fixed Qwen3-Max dispatch}%
\newlength{\policygap}\setlength{\policygap}{0.42cm}%
\newlength{\policypanelw}%
\newlength{\policylabsep}\setlength{\policylabsep}{4pt}% label shift; the 2.5pt tick length adds to it
\newlength{\policylabgap}\setlength{\policylabgap}{\dimexpr\policylabsep+2.5pt\relax}%
\setlength{\policypanelw}{\dimexpr(\linewidth-\policylabelw-\policylabgap-2\policygap)/3\relax}%
% Rows bottom to top, with half-row gaps between the four policy groups.
\def\yOpus{1}\def\yOracle{2}%
\def\yACR{3.5}\def\yCascade{4.5}\def\yQwen{5.5}%
\def\yQC{7}\def\yPred{8}%
\def\yEpsA{9.5}\def\yEpsZ{10.5}\def\yUnc{11.5}%
% Group bands, drawn in every panel at the same heights.
\newcommand{\policybands}[2]{%
  \path[fill=policyblue!6] (axis cs:#1,9.0) rectangle (axis cs:#2,12.0);
  \path[fill=policyteal!8] (axis cs:#1,6.5) rectangle (axis cs:#2,8.5);
  \path[fill=black!3.5] (axis cs:#1,3.0) rectangle (axis cs:#2,6.0);
  \path[fill=black!3.5] (axis cs:#1,0.5) rectangle (axis cs:#2,2.5);}%
\pgfplotsset{
  policyaxis/.style={
    scale only axis,width=\policypanelw,height=5.3cm,
    ymin=0.5,ymax=12.0,
    ytick={\yOpus,\yOracle,\yACR,\yCascade,\yQwen,\yQC,\yPred,\yEpsA,\yEpsZ,\yUnc},
    yticklabels={},
    axis x line*=bottom,axis y line*=left,
    tick align=outside,xtick pos=bottom,
    major tick length=2.5pt,
    tick label style={font=\footnotesize,text=black!75},
    xticklabel style={yshift=1pt},
    label style={font=\footnotesize,text=black!85},
    xlabel style={yshift=2pt},
    title style={font=\footnotesize\bfseries,yshift=-2pt},
    xmajorgrids,major grid style={black!9,line width=0.4pt},
    axis line style={black!35},
    y axis line style={draw=none},
    ytick style={draw=none},
    axis on top=false,
    clip=false,
  },
  policydot/.style={only marks,mark=*,mark size=2.1pt,mark options={draw=white,line width=0.35pt}},
  policyinterval/.style={
    policydot,
    error bars/.cd,x dir=both,x explicit,
    error bar style={line width=0.8pt},
    error mark options={rotate=90,mark size=2pt,line width=0.6pt},
    /pgfplots/.cd,
  },
  policyref/.style={black!45,dashed,line width=0.55pt,forget plot},
}%
\begin{tikzpicture}
\begin{axis}[policyaxis,name=efficiency,
  yticklabels={Always-Opus,
    Per-task oracle,
    ACRouter map,
    Best fixed cascade,
    Fixed Qwen3-Max dispatch,
    Quality-cost router,
    {Predicted 21 cells, $\epsilon=0$},
    {21 cells, $\epsilon=0.01$},
    {21 cells, $\epsilon=0$},
    {21 cells, unconstrained}},
  yticklabel style={font=\footnotesize,text=black!85,align=right,inner xsep=0pt,
    text height=1.7ex,text depth=0.45ex},
  yticklabel shift=\policylabsep,
  xmode=log,log basis x=10,xmin=0.75,xmax=48,
  xtick={1,3,10,30},xticklabels={1,3,10,30},
  error bars/error mark=none,
  title={Dollar efficiency},xlabel={$\eta/\eta_B$ (log scale)}]
\policybands{0.75}{48}
\addplot[policyref] coordinates {(1,0.5) (1,12)};
\addplot[policyinterval,color=policyblue] coordinates {
  (28.187,\yUnc) += (1.472,0) -= (1.347,0)
  (25.516,\yEpsZ) += (1.387,0) -= (1.238,0)
  (27.612,\yEpsA) += (1.460,0) -= (1.301,0)
};
\addplot[policyinterval,color=policyteal] coordinates {
  (25.324,\yPred) += (1.326,0) -= (1.227,0)
  (24.166,\yQC) += (1.415,0) -= (1.305,0)
};
\addplot[policyinterval,color=policyslate] coordinates {
  (20.097,\yQwen) += (1.200,0) -= (1.132,0)
  (2.004,\yCascade) += (0.136,0) -= (0.123,0)
  (1.745,\yACR) += (0.081,0) -= (0.079,0)
};
\addplot[policyinterval,color=policyamber,mark=diamond*,mark size=2.7pt]
  coordinates {(33.510,\yOracle) += (1.696,0) -= (1.445,0)};
\addplot[only marks,mark=square*,mark size=1.9pt,color=black!70]
  coordinates {(1,\yOpus)};
\end{axis}
\begin{axis}[policyaxis,at={(efficiency.south east)},anchor=south west,xshift=\policygap,
  name=cost,
  xmode=log,log basis x=10,xmin=0.25,xmax=17,
  xtick={0.3,1,3,10},xticklabels={0.3,1,3,10},
  title={Cost per task},xlabel={m\$ (log scale)}]
\policybands{0.25}{17}
\addplot[policyref] coordinates {(11.655,0.5) (11.655,12)};
\addplot[policydot,color=policyblue]
  coordinates {(0.395,\yUnc) (0.452,\yEpsZ) (0.409,\yEpsA)};
\addplot[policydot,color=policyteal]
  coordinates {(0.453,\yPred) (0.482,\yQC)};
\addplot[policydot,color=policyslate]
  coordinates {(0.525,\yQwen) (6.556,\yCascade) (7.643,\yACR)};
\addplot[only marks,mark=diamond*,mark size=2.7pt,color=policyamber,mark options={draw=white,line width=0.35pt}]
  coordinates {(0.368,\yOracle)};
\addplot[only marks,mark=square*,mark size=1.9pt,color=black!70]
  coordinates {(11.655,\yOpus)};
\end{axis}
\begin{axis}[policyaxis,at={(cost.south east)},anchor=south west,xshift=\policygap,
  name=quality,
  xmin=-0.068,xmax=0.085,scaled x ticks=false,
  xtick={-0.05,0,0.05},xticklabels={$-0.05$,$0$,$+0.05$},
  minor xtick={-0.025,0.025,0.075},minor tick length=0pt,
  minor grid style={black!5,line width=0.4pt},xminorgrids,
  title={Quality change},xlabel={Mean score, $\Delta V$}]
\policybands{-0.068}{0.085}
\addplot[policyref] coordinates {(0,0.5) (0,12)};
\addplot[policyinterval,color=policyblue] coordinates {
  (-0.0201,\yUnc) += (0.0145,0) -= (0.0142,0)
  (-0.0044,\yEpsZ) += (0.0141,0) -= (0.0131,0)
  (-0.0140,\yEpsA) += (0.0136,0) -= (0.0132,0)
};
\addplot[policyinterval,color=policyteal] coordinates {
  (-0.0070,\yPred) += (0.0137,0) -= (0.0130,0)
  (-0.0003,\yQC) += (0.0135,0) -= (0.0135,0)
};
\addplot[policyinterval,color=policyslate] coordinates {
  (-0.0416,\yQwen) += (0.0141,0) -= (0.0133,0)
  (0.0558,\yCascade) += (0.0102,0) -= (0.0097,0)
  (0.0631,\yACR) += (0.0100,0) -= (0.0103,0)
};
\addplot[policyinterval,color=policyamber,mark=diamond*,mark size=2.7pt]
  coordinates {(0.0248,\yOracle) += (0.0128,0) -= (0.0131,0)};
\addplot[only marks,mark=square*,mark size=1.9pt,color=black!70]
  coordinates {(0,\yOpus)};
\end{axis}
% Bounding box = label column + panels, so the figure spans exactly \linewidth.
\pgfresetboundingbox
\path[use as bounding box]
  ([xshift=-\policylabelw-\policylabgap]efficiency.outer south west -| efficiency.west)
  rectangle (quality.outer north east -| quality.east);
\end{tikzpicture}%
\endgroup%

==> fig/robot-condition.tex <==
% RoboTwin test scenes (1,000 clean, 1,000 randomized): success of the two strongest
% policies, the outcome router, and the per-scene oracle (left); mean policy seconds (right).
\begingroup
\definecolor{vizblue}{HTML}{2A78D6}%
\definecolor{vizorange}{HTML}{EB6834}%
\definecolor{vizaqua}{HTML}{1BAF7A}%
\definecolor{vizink}{HTML}{0B0B0B}%
\definecolor{vizmuted}{HTML}{52514E}%
\pgfplotsset{
  robotaxis/.style={
    scale only axis,axis x line*=bottom,axis y line*=left,
    tick align=outside,
    tick label style={font=\scriptsize,text=vizmuted},
    label style={font=\scriptsize,text=vizmuted},
    axis line style={black!35},
    clip=false,
  },
}%
\begin{tikzpicture}
\begin{axis}[robotaxis,name=success,width=5.2cm,height=2.6cm,
  ybar=1.5pt,bar width=0.40cm,ymin=0,ymax=100,ytick={0,25,50,75,100},
  ymajorgrids,major grid style={black!9},xtick style={draw=none},
  symbolic x coords={Clean,Randomized},xtick=data,enlarge x limits=0.42,
  x tick label style={font=\scriptsize,text=vizink},
  ylabel={Success (\%)},ylabel style={yshift=-4pt},
  title={Success by scene condition},title style={font=\scriptsize\bfseries,text=vizink,yshift=-2pt},
  legend style={at={(1.08,0.5)},anchor=west,legend columns=1,draw=none,fill=none,
    font=\scriptsize,text=vizink,row sep=1pt,cells={anchor=west}},
  legend image code/.code={\fill[#1] (0cm,-0.07cm) rectangle (0.22cm,0.11cm);}]
\addplot[fill=vizorange,draw=none] coordinates {(Clean,78.4) (Randomized,62.5)};
\addplot[fill=vizaqua,draw=none] coordinates {(Clean,81.7) (Randomized,45.6)};
\addplot[fill=vizblue,draw=none] coordinates {(Clean,81.6) (Randomized,61.5)};
\legend{ME-Dex (fixed),PatchWAM,Router}
\draw[black!50,dashed,line width=0.6pt] ([xshift=-0.66cm]axis cs:Clean,93.3) -- ([xshift=0.66cm]axis cs:Clean,93.3)
  node[right,font=\tiny,text=vizmuted,inner sep=1pt] {oracle};
\draw[black!50,dashed,line width=0.6pt] ([xshift=-0.66cm]axis cs:Randomized,84.4) -- ([xshift=0.66cm]axis cs:Randomized,84.4);
\end{axis}
\begin{axis}[robotaxis,at={(success.south east)},anchor=south west,xshift=4.3cm,
  width=4.2cm,height=2.0cm,
  xbar=0pt,bar shift=0pt,bar width=0.24cm,xmin=0,xmax=16,xtick={0,4,8,12,16},
  xmajorgrids,major grid style={black!9},
  y axis line style={draw=none},ytick style={draw=none},
  ymin=0.5,ymax=3.5,ytick={1,2,3},yticklabels={Router,PatchWAM,ME-Dex},
  yticklabel style={font=\scriptsize,text=vizink},
  xlabel={Mean policy time per scene (s)},xlabel style={yshift=3pt},
  title={Policy time},title style={font=\scriptsize\bfseries,text=vizink,yshift=-2pt},
  nodes near coords={\pgfmathprintnumber[fixed,fixed zerofill,precision=2]{\pgfplotspointmeta}},
  nodes near coords style={font=\tiny,text=vizink,inner sep=1.5pt},
  point meta=x]
\addplot[fill=vizblue,draw=none] coordinates {(11.05,1)};
\addplot[fill=vizaqua,draw=none] coordinates {(11.10,2)};
\addplot[fill=vizorange,draw=none] coordinates {(14.51,3)};
\end{axis}
\end{tikzpicture}%
\endgroup


==> fig/verifier-comparison.tex <==
\begingroup
\definecolor{verifierblue}{HTML}{3568A8}
\definecolor{verifierorange}{HTML}{C77C2B}
\resizebox{0.92\textwidth}{!}{%
\begin{tikzpicture}
\begin{groupplot}[
  group style={group size=2 by 1,horizontal sep=0.75cm},
  height=4.2cm,width=8.5cm,
  ymin=0.5,ymax=5.5,ytick={1,2,3,4,5},
  yticklabels={Released-score oracle,LLM judge (proxy price),Hidden tests,Visible examples,Compiler},
  tick label style={font=\small},label style={font=\small},
  title style={font=\normalsize},tick align=outside,
  axis line style={black!70},xmajorgrids,
  major grid style={black!12},
  legend style={draw=none,fill=none,font=\small,at={(0.99,0.5)},anchor=east,legend columns=1,
    /tikz/every even column/.append style={column sep=0.3cm}},
  legend cell align=left
]
\nextgroupplot[title={Efficiency including verifier cost},
  xmode=log,xmin=0.4,xmax=25,xtick={0.5,1,2,5,10,20},
  log ticks with fixed point,
  xlabel={Relative dollar efficiency, $\eta/\eta_B$}]
\addplot[black!55,dashed,forget plot] coordinates {(1,0.5) (1,5.5)};
\addplot[only marks,mark=*,mark size=2.3pt,color=verifierblue,
  error bars/.cd,x dir=both,x explicit]
  coordinates {
    (1.98,4.13) += (0.37,0) -= (0.26,0)
    (2.87,3.13) += (0.66,0) -= (0.49,0)
    (1.09,2.13) += (0.12,0) -= (0.09,0)
    (2.46,1.13) += (0.47,0) -= (0.37,0)
    (4.09,5.13) += (1.36,0) -= (0.86,0)
  };
\addlegendentry{$\theta=0.5$}
\addplot[only marks,mark=square*,mark size=2.3pt,color=verifierorange,
  error bars/.cd,x dir=both,x explicit]
  coordinates {
    (1.06,3.87) += (0.04,0) -= (0.03,0)
    (2.37,2.87) += (0.43,0) -= (0.34,0)
    (0.64,1.87) += (0.02,0) -= (0.03,0)
    (2.46,0.87) += (0.47,0) -= (0.37,0)
    (4.09,4.87) += (1.36,0) -= (0.86,0)
  };
\addlegendentry{$\theta=1$}
\nextgroupplot[title={Quality at $\theta=0.5$},width=5.4cm,
  xmin=-0.07,xmax=0.095,xtick={-0.05,0,0.05},
  yticklabels={},xlabel={Mean score change, $Q$},
  scaled x ticks=false,
  xticklabel style={/pgf/number format/fixed,/pgf/number format/precision=2}]
\addplot[black!55,dashed] coordinates {(0,0.5) (0,4.5)};
\addplot[only marks,mark=*,mark size=2.7pt,color=verifierblue,
  nodes near coords,point meta=explicit symbolic,
  every node near coord/.append style={font=\scriptsize,anchor=west,xshift=1.5pt}]
  coordinates {(-0.036,4) [$-0.036$] (0.024,3) [$+0.024$]
    (-0.012,2) [$-0.012$] (0.045,1) [$+0.045$]
    (-0.024,5) [$-0.024$]};
\end{groupplot}
\end{tikzpicture}%
}
\endgroup

